A proposal for community driven and decentralized astronomical databases and the Open Exoplanet Catalogue

I present a new kind of astronomical database based on small text files and a distributed version control system. This encourages the community to work collaboratively. It creates a decentralized, completely open and democratic way of managing small to medium sized heterogeneous astronomical databases and catalogues. The use of the XML file format allows an easy to parse and read, yet dynamic and extendable database structure. The Open Exoplanet Catalogue is based on these principles and presented as an example. It is a catalogue of all discovered extra-solar planets. It is the only catalogue that can correctly represent the orbital structure of planets in arbitrary binary, triple and quadruple star systems, as well as orphan planets.

==> Makefile <==
# This file generates files required to use the listings package.
#
# (c) 2007 Brooks Moses
#
# This file is distributed under the terms of the LaTeX Project Public
# License from CTAN archives in directory  macros/latex/base/lppl.txt.
# Either version 1.3 or, at your option, any later version.

.PHONY: listings pdf pdf-devel all

listings: listings.sty

pdf: listings.pdf

pdf-devel: listings-devel.pdf

all: listings pdf pdf-devel


listings.sty: listings.dtx listings.ins lstdrvrs.dtx
	tex listings.ins

listings.pdf: listings.sty
	rm -f ltxdoc.cfg
	pdflatex listings.dtx
	makeindex -s gind.ist listings
	pdflatex listings.dtx
	pdflatex listings.dtx

listings-devel.pdf: listings.sty
	rm -rf ltxdoc.cfg
	echo "\AtBeginDocument{\AlsoImplementation}" > ltxdoc.cfg
	pdflatex -jobname=listings-devel listings.dtx
	makeindex -s gind.ist listings-devel
	pdflatex -jobname=listings-devel listings.dtx
	pdflatex -jobname=listings-devel listings.dtx
	rm -rf ltxdoc.cfg

